On the Consistency of Video Large Language Models in Temporal Comprehension

Video large language models (Video-LLMs) can temporally ground language queries and retrieve video moments. Yet, such temporal comprehension capabilities are neither well-studied nor understood. So we conduct a study on prediction consistency -- a key indicator for robustness and trustworthiness of temporal grounding. After the model identifies an initial moment within the video content, we apply a series of probes to check if the model's responses align with this initial grounding as an indicator of reliable comprehension. Our results reveal that current Video-LLMs are sensitive to variations in video contents, language queries, and task settings, unveiling severe deficiencies in maintaining consistency. We further explore common prompting and instruction-tuning methods as potential solutions, but find that their improvements are often unstable. To that end, we propose event temporal verification tuning that explicitly accounts for consistency, and demonstrate significant improvements for both grounding and consistency. Our data and code are open-sourced at https://github.com/minjoong507/Consistency-of-Video-LLM.

==> secs/sup.tex <==
\clearpage
\maketitlesupplementary
\setcounter{page}{1}
\setcounter{section}{0}
\appendix

In this file, we provide additional details as follows:

\begin{enumerate}[label=\Alph*.]
    \item \textbf{Details of Evaluation Datasets}: We provide the details of our proposed datasets, Charades-CON and ActivityNet-CON.

    \item \textbf{Details of Models}: We describe the \vllm~that are utilized in our experiments one by one. Then we provide the experiment setup of the models for our evaluation. Additionally, we further discuss the limitations of the time-aware models.

    \item \textbf{Details of Prompting Methods}: We describe two prompting methods, including chain-of-thought and description prompting.
    
    \item \textbf{Details of Instruction Tuning}: We detail the process of instruction tuning and \method.

    \item \textbf{Additional Experiments}: We provide additional experiments to provide further insights.

    \item \textbf{Prompt Designs}: In this study, we design various prompts to construct evaluation sets, evaluate the model's responses, and generate verification queries. We provide detailed prompts for each.
\end{enumerate}

\section{Details of Datasets}
In Table~\ref{tbl: dataset_details}, we provide statistics of each dataset. The length of the video and their moments remain almost the same compared to the original datasets. Generated aligned and misaligned queries have similar lengths compared to the ground-truth queries. 

\section{Details of \vllm}
\label{appendix: model details}
\subsection{\vllm}
\label{appendix: explanation of vllms}
In this section, we describe eight open-source \vllm: Video-LLaMA~\cite{videollama}, Video-LLaVA~\cite{lin2023videollava}, Video-ChatGPT~\cite{Maaz2023VideoChatGPT}, VideoChat2~\cite{li2024mvbench}, Video-LLaMA2~\cite{cheng2024videollama2}, TimeChat~\cite{timechat}, VTimeLLM~\cite{vtimellm}, and VTG-LLM~\cite{guo2024vtgllm}, which are utilized in our evaluation. Note that we experiment with a single A100 GPU for all models.

\begin{enumerate}
\item \textbf{Video-LLaMA} exhibits two branches: Vision-Language and Audio-Language in its modeling and utilizes cross-modal training from both the frozen pre-trained visual and audio encoder. It shows a remarkable zero-shot audio understanding capability and also generates responses to the visual and audio information presented in the videos. We select the fine-tuned checkpoint: \textit{Video-LLaMA-2-7B-Finetuned}, which is additionally fine-tuned on the instruction tuning data from Mini-GPT-4~\cite{zhu2023minigpt}, LLaVA~\cite{liu2023llava}, and VideoChat~\cite{li2023videochat}.
% released at \url{https://github.com/DAMO-NLP-SG/Video-LLaMA}

\item \textbf{Video-LLaVA} enables an LLM to perform visual reasoning capabilities, and it leads to comprehending both images and videos simultaneously. To do this, Video-LLaVA collects both image and video-text datasets and incorporates them in its instruction tuning. 
% We utilize the official checkpoint released at \url{https://github.com/PKU-YuanGroup/Video-LLaVA}.

\item \textbf{Video-ChatGPT} designs spatiotemporal video modeling and constructs video instruction tuning upon LLaVA~\cite{liu2023llava}. It introduces a new dataset for video instruction tuning, containing 100,000 high-quality video-instruction pairs. Video-ChatGPT outperforms previous \vllm ~in Zero-shot VQA across several benchmarks. Additionally, Video-ChatGPT proposes a video conversation evaluation framework. 
% We use the checkpoint released at \url{https://github.com/mbzuai-oryx/Video-ChatGPT}.
\begin{figure}[t]
        \centering
        \includegraphics[width=0.99\linewidth]{appendix_figures/prompt_results2.pdf}
    \caption{
    Consistency evaluation results of Video-ChatGPT and VideoChat2 using different prompting methods. While the prompting methods improve Video-ChatGPT, they are ineffective for VideoChat2.
    }
    \label{fig: prompt results for Video-ChatGPT and VideoChat2}
\end{figure}
\input{appendix_tables/dataset_details}
\input{appendix_tables/templates_for_holistic verification}

\item \textbf{VideoChat2} design a progressive multimodal training. Specifically, they aim to align vision and text in the first stage and then generate captions from various image-text pairs. Finally, they conduct instruction tuning to better align responses with human instructions. VideoChat2 demonstrates significant improvements in Zero-Shot Video Question Answering, video conversation, and own built comprehensive video benchmarks. 
% We use the checkpoint released at \url{https://github.com/OpenGVLab/Ask-Anything/tree/main/video_chat2}.

\item \textbf{Video-LLaMA2} is one of the state-of-the-art \vllm, demonstrating superior performances on video question-answering tasks. They seamlessly integrate both visual and audio modalities in videos and propose STC connector to understand spatiotemporal video information. 
% We use the checkpoint released at \url{https://github.com/DAMO-NLP-SG/VideoLLaMA2}.
\input{appendix_tables/grounding_templates}

\item \textbf{TimeChat} is specifically developed to accurately localize and understand specific video moments from long videos. TimeChat designs two key architectural: (1) A time-aware frame encoder that explicitly encodes video frames along with timestamps, (2) A sliding video Q-Former to accommodate sequential information in video frames. Specifically, TimeChat borrows the image Q-Former from InstructBLIP~\cite{dai2023instructblip} and the video Q-former from Video-LLaMA~\cite{videollama}. Additionally, TimeChat includes the instruction tuning datasets of Valley~\cite{luo2023valley} and constructs 125K video instruction tuning datasets to perform time-related video understanding tasks, such as VTG and DVC. 
% We use the checkpoint released at \url{https://github.com/RenShuhuai-Andy/TimeChat}.

\item \textbf{VTimeLLM} proposes a three-stage temporal-aware method, including image-text training and understanding events within the video, enabling more precise video temporal understanding. VTimeLLM devises two types of QA dialogue templates, including single-turn and multi-turn, to prompt questions requiring a comprehensive description of all events and their corresponding timestamps. 
% We use the checkpoint released at \url{https://github.com/huangb23/VTimeLLM}.

\item \textbf{VTG-LLM} utilizes specific modules to improve temporal representations in Video-LLM. While previous \vllm~suffer quantization errors by using special time tokens, VTG-LLM use absolute-time tokens (\eg, \text{<TIME$\_$ZERO>, <TIME$\_$ONE>}) to resolve this and handle videos more than one hour. The model is instruction-tuned with VTG-IT-120K,  a high-quality and comprehensive instruction tuning for time-related video understanding tasks. 
% We use the checkpoint released at \url{https://github.com/gyxxyg/VTG-LLM}. 
\end{enumerate}
\input{appendix_tables/grounding_results}
\input{appendix_tables/grounding_GPT4o}

\subsection{Evaluation Setup}
\label{appendix: evaluation setup}
As previously mentioned in Section~\ref{sec: experiments}, the feasibility of general-purpose \vllm~and closed-source models for temporal grounding is absent. In this section, we provide adaptation details for these models. 

\noindent\textbf{General-purpose \vllm.} We empirically found that the general-purpose \vllm~are very sensitive to prompts, easily failing to extract timestamps from their answers. For instance, the model does not meet our expectations, such as answering ``I'm unable to find timestamps in the video'', or the model's answer only includes a single timestamp like ``The given event happens at 3 seconds.'' We categorize these answers as \textit{Invalid output}. Therefore, we carefully design several prompts for temporal grounding to find the stable setting for each model and provide experiment results in Table~\ref{tbl: finding the optimal setting for temporal grounding}. For Video-LLaMA, we have two options for LLM backbones, Llama-2 and Vicuna. While using LLaMA-2 as an LLM backbone and the first prompt achieves the best grounding performance, it demonstrates unstable performance depending on the prompt. Therefore, we utilize Vicuna and the first prompt (\ie, [1] in Table~\ref{tbl: grounding prompt templates}), demonstrating better consistency (see Table~\ref{tbl: consistency of vllm across different settings}). Other \vllm~like Video-ChatGPT are fixed with a specific LLM backbone, so we follow their development settings. 
% We choose the first prompt for VideoChat2 and the third prompt for Video-LLaVA, Video-ChatGPT, and Video-LLaMA2. 
In conclusion, we use the first prompt for Video-LLAMA and VideoChat2, the second prompt for Video-LLAVA, and the third prompt for Video-ChatGPT and VideoLLaMA2.
\begin{figure*}[t]
        \centering
        \includegraphics[width=0.99\linewidth]{prompt_figures/CoT.pdf}
    \caption{
    Chain-of-Thought prompts for temporal grounding and the probes. Since temporal grounding, rephrased grounding, and shifted grounding share the same goal, predicting the video moment accurately, they use the same prompt. For verification probes, we specify which parts the model should focus on, whether it’s the entire sentence or specific sub-elements.
    }
    \label{fig: COT prompts}
\end{figure*}

\begin{figure}[t]
        \centering
        \includegraphics[width=0.99\linewidth]{appendix_figures/Desc.pdf}
    \caption{
    The responses of Video-ChatGPT with Description prompting. While Video-ChatGPT generates a rich video caption, it contains incorrect information that may mislead accurate predictions. In this case, Video-ChatGPT fails to accurately predict the timestamp in the video.
    }
    \label{fig: description prompts}
\end{figure}

\noindent\textbf{Time-aware \vllm.} For TimeChat, VTimeLLM, and VTG-LLM, we follow the same prompt templates, which are used in their official instruction tuning for temporal grounding. Likewise, we use the official codes to extract the timestamps from their predictions.

\noindent\textbf{Closed-source Models.} Given the considerable budget required to utilize GPT-4o, we first define the set of frame numbers \{10, 32, 64\} and sub-sample 100 videos from each dataset to efficiently find the optimal setting. In Table~\ref{tbl: GPT-4o grounding}, we provide the grounding performance of GPT-4o across different frame numbers. Note that the performances in Table~\ref{tbl: GPT-4o grounding} are different from those in Table~\ref{tbl: consistency} because the number of test samples is different. During the experiment, we instruct GPT-4o on how many frames are in the given video and how long each frame is sampled. We find that using 10 frames shows the best performance. For Gemini, we use the official APIs to process video inputs.

\noindent\textbf{Visualization.} We present example question-answer pairs for all models in Table~\ref{tbl: qa examples}. The format of timestamps varies depending on the model, so we design a timestamp extraction function for each model.


\subsection{Limitations of the Time-aware Models}
\label{appendix: limitations of the time-aware models}
We hypothesize that the excessive focus on temporal grounding with specialized elements in the time-aware models may limit its adaptability to various video understanding tasks and hinder generalization capabilities. For instance, TimeChat develops a time-aware frame encoder that explicitly encodes video features along with the corresponding sentences containing timestamps, such as ``This frame is sampled at 2s.'' VTG-LLM utilizes digit time tokens, such as \text{<TIME$\_$ZERO> and <TIME$\_$ONE>}, to effectively represent timestamps in videos. While such methods may be effective for answering questions that require timestamps within videos, providing these timestamp priors could hinder generalization across various video understanding tasks. This limitation is particularly evident in VTG-LLM, which shows poor relative consistency for verification probes, and we empirically find that VTG-LLM often struggles to follow instructions. Specifically, VTG-LLM frequently generates timestamps as answers, even when asked for verification probes.
\section{Details of Prompting Methods}
\label{appendix: prompting methods}
In this section, we provide details of the two prompting methods, Chain-of-Thought and Description prompting.

\noindent\textbf{Chain-of-Thought.} We provide prompts that we utilize for each prompting method. In Figure~\ref{fig: COT prompts}, we give three chain-of-thought prompts that we design for each probe in our evaluation. The three tasks, temporal grounding, rephrased grounding, and shifted grounding, share the same prompt since their output is the same. For holistic and compositional verification, we instruct on which part the model should concentrate either a whole sentence or sub-elements.

\noindent\textbf{Description Prompting.} We first ask the model ``Please describe the given video in detail.'' Then we keep the generated video description in chat history to perform the probes during our evaluation. We give a visual example of Video-ChatGPT using the description prompting method in Figure~\ref{fig: description prompts}. In our previous discussion, we highlighted that while using the description prompting method enhances the model's consistency, it may lead to negative outcomes such as generating incorrect descriptions or hallucinations. As illustrated in Figure~\ref{fig: description prompts}, Video-ChatGPT provides a detailed description of the video, but some of the information in the generated description is inaccurate. For instance, the video depicts two men in a gym, with only one of them wearing a red shirt. However, the model incorrectly states that both men are wearing red shirts. This might lead to inaccurate moment predictions.

\section{Details of Instruction Tuning}
\label{appendix: instruction tuning}
In this section, we provide a detailed experiment setup for instruction tuning and \method.

\noindent\textbf{Instruction Tuning.} Following the previous work~\cite{timechat}, we collect the annotations in the train split and convert the annotations into a task-specific template to derive \vllm~can predict the timestamps. For example, if the query ``The person closes the laptop.'' is grounded in 0 to 5 seconds in the video, we prompt the models ~``Localize the visual content described by the given textual query `The person closes the laptop.' in the video, and output the start and end timestamps in seconds.''. Then the model's answer should be ``The given query happens in 0 - 5 seconds.'' We utilize the official codes and configurations to conduct instruction tuning upon their official checkpoints. 
\input{appendix_tables/grounding_with_IoUs}

\noindent\textbf{Event Temporal Verification Tuning.} We construct verification questions from the training split of each dataset. Specifically, we generate both aligned and misaligned sentences from the original query and also generate correction information on what information is wrong in misaligned sentences by providing the prompt in Figure~\ref{fig: prompt for ETVT} to GPT-4o-mini. Then we pair aligned sentences with affirmative responses and misaligned sentences with denial responses and their corresponding corrections.

\noindent\textbf{Experiment Settings.} The number of queries by type for each dataset can be found in Table~\ref{tbl: the number of queries}. For \method, we follow the official configurations and only change the parameters, including iters per epoch and warmup steps, to reflect the number of annotations for each training. We report hyper-parameters used in each instruction tuning method in Table~\ref{tbl: hyperparameters}. We use 4$\times$80 GB A100 GPUs for all experiments and use the same prompts and hyper-parameters in both Video-LLaMA and TimeChat. In our setting, Video-LLaMA requires less than one day, and TimeChat requires at least two days for instruction tuning. For \method, Video-LLaMA takes under two days, while TimeChat requires six days.
\input{appendix_tables/hyperparameters}
\input{appendix_tables/statistics of queries}
\input{appendix_tables/consistency_across_different_prompts}
\input{appendix_tables/rephrased_grounding}

\section{Additional Experiments}
\label{appendix: additional experiments}
In this section, we provide additional experiment results to further provide insights. We first provide the consistency evaluation results using different IoU values. Then we examine how the prompt for temporal grounding and scalability of LLM impact consistency. Then we further analyze the results of rephrased grounding and shifted grounding.

% \subsection{The impact of Prompt Designs and Scalability of LLM on Consistency.} 
\noindent\textbf{Consistency Results across Different IoU thresholds.} In Table~\ref{tbl: grounding and consistency across different IoUs}, we provide additional experiment results using an additional IoU threshold (\ie, 0.7) for temporal grounding and grounding probes.

\noindent\textbf{The impact of Temporal Grounding Prompt on Consistency.} 
\label{appendix: impact of prompt and LLM scale}
To investigate this, we provide the results in Table~\ref{tbl: consistency of vllm across different settings}. As the prompt designs affect the grounding performance of \vllm, we also investigate their consistency. Specifically, we select a series of settings that demonstrate high performance for each model in Table~\ref{tbl: finding the optimal setting for temporal grounding}. While Video-LLaMA with Vicuna-7B and the second prompt demonstrate better relative consistency scores for verification probes, there is no significant performance gap compared to other settings. Likewise, for Video-LLaVA, Video-ChatGPT, and Video-LLaMA2, the grounding prompt does not significantly impact the model's performance.

\noindent\textbf{The impact of Scalability of LLM on Consistency.} Additionally, we evaluate Video-LLaMA with Vicuna-13B and confirm that there are no significant improvements. Specifically, while it shows higher relative consistency in rephrased grounding, it fails to demonstrate strong capabilities for other probes. Likely, a larger-scale LLM does not necessarily represent improved consistency. Unfortunately, we cannot evaluate the models with larger-scale LLM backbones, as most of them have either conducted experiments only with 7B LLMs or have not released the corresponding checkpoints. For instance, TimeChat and VTG-LLM haven't officially conducted experiments using 13B LLM backbones. VTimeLLM reports the performance using Vicuna-13B in the original paper, but has not officially released the corresponding checkpoint.

\noindent\textbf{Analysis of Rephrased Grounding.} In Table~\ref{tbl: mIoU of rephrased grounding}, we provide the performance for rephrased grounding by three modification rules. The rules are previously introduced in~\Cref{sec: dataset} including word replacement, active-to-passive conversion, and word order change. We confirm that most models temporally ground rephrased queries with word replacement. 
As we discussed in~\Cref{sec: experiments}, this suggests the need for improvements in consistent grounding and demonstrates the effectiveness of our modification rules providing various language variations.

\noindent\textbf{How does VTune improve grounding?} We speculate that VTune enhances grounding in multiple ways. Fig~\ref{appendix: VTune}-(A) shows that verification tuning alone improves grounding performance by approximately 20\% (from an initial 30.5), suggesting that verification tasks inherently benefit grounding. This is likely because verification tasks are more general and align with the prior QA capabilities of LLMs, whereas fine-tuning for grounding may override this knowledge due to requiring task-specific timestamp templates, resulting in poor consistency. Additionally, Fig~\ref{appendix: VTune}-(B) highlights the importance of dataset scale and diversity, indicating that verification queries serve as effective data augmentation, expanding linguistic coverage. However, excessive training may diminish performance.

\begin{figure}[t]
        \centering
        \includegraphics[width=0.99\linewidth]{appendix_figures/VTune.pdf}
    \caption{
    \textbf{Experiments on Charades-CON with TimeChat.} \textbf{(A)}: Performance evaluation across different ratios of event and temporal verification queries. The total queries are fixed at 12k, matching the \# of grounding queries in the original dataset.
    \textbf{(B)}: Performance evaluation across varying verification query scales. 100\% scale corresponds to the performance of VTune reported in the paper. The number of unique words is a proxy for dataset diversity.
    }
    \label{appendix: VTune}
\end{figure}

\begin{figure*}[t]
        \centering
        \includegraphics[width=0.99\linewidth]{prompt_figures/VTune.pdf}
    \caption{
    The prompt to generate verification questions for \method.
    }
    \label{fig: prompt for ETVT}
\end{figure*}

\begin{figure*}[t]
        \centering
        \includegraphics[width=0.99\linewidth]{prompt_figures/datasets.pdf}
    \caption{
    The prompt for generating aligned, misaligned, and compositional queries.
    }
    \label{fig: prompt to construct evaluation sets}
\end{figure*}

\begin{figure*}[t]
        \centering
        \includegraphics[width=0.99\linewidth]{prompt_figures/evaluation.pdf}
    \caption{
    The prompt to assess the correctness of the model's answer for verification probes. Specifically, we ask GPT-4o-mini to assess whether the answer aligns with the expected answer.}
    \label{appendix_fig: prompt for evaluation}
\end{figure*}

\section{Prompts for GPT}
\label{appendix: prompt designs}
In this section, we provide detailed prompts that are utilized in our study.
\begin{enumerate}
    \item We use the prompt in Figure~\ref{fig: prompt to construct evaluation sets} to generate aligned, misaligned, and compositional queries.

    \item We use the prompt in Figure~\ref{appendix_fig: prompt for evaluation} to evaluate the model's answer for our probes.
\end{enumerate}
\input{appendix_tables/qa_examples}
